Limits on atomic qubit control from laser noise

Technical noise present in laser systems can limit their ability to perform high fidelity quantum control of atomic qubits. The ultimate fidelity floor for atomic qubits driven with laser radiation is due to spontaneous emission from excited energy levels. The goal is to suppress the technical noise from the laser source to below the spontaneous emission floor such that it is no longer a limiting factor. It has been shown that the spectral structure of control noise can have a large influence on achievable control fidelities, while prior studies of laser noise contributions have been restricted to noise magnitudes. Here, we study the unique spectral structure of laser noise and introduce a new metric that determines when a stabilised laser source has been optimised for quantum control of atomic qubits. We find requirements on stabilisation bandwidths that can be orders of magnitude higher than those required to simply narrow the linewidth of a laser. We introduce a new metric, the $\chi$-separation line, that provides a tool for the study and engineering of laser sources for quantum control of atomic qubits below the spontaneous emission floor.

==> OldText.tex <==
The laser has become an invaluable tool in the control of atomic systems due to fine structure atomic transitions typically having optical wavelengths. The application of atoms to the fields of frequency standards and quantum information has necessitated the use of ultra-stable local oscillators (LOs) generated from laser radiation. The demonstration of an optical clock in Al$^+$ with fractional stabilities $<10^{-18}$ highlights in part the level of atomic control now possible with laser radiation \cite{brewer2019al+}. In the field of quantum information, laser-driven single qubit rotations have been performed with average errors on the level of $10^{-4}$ \cite{ballance2016high}. To further improve on these metrics it is pertinent to student the influence of the local oscillator noise on the controllability of atomic states. The identification of the important contributions to control errors from laser noise will enable the design and engineering of laser systems for high-fidelity control. Such a study has been performed for microwave LOs \cite{ball2016role}, where it was found that both the magnitude and spectral structure of the LO phase noise were critical influences on single-qubit gate fidelities. In this study we outline the typical magnitude and spectral structure present in local oscillators derived from laser radiation, and calculate the dependence of atomic qubit fidelities on these noise fields.

Atomic qubits are typically encoded in states separated by either optical or microwave transition frequencies (see Figure \ref{fig:overview}). For optical transitions, narrow-linewidth laser radiation can be directly used to coherently rotate the qubit state. For microwave transitions, a microwave beatnote can be generated from two phase-coherent optical frequencies offset by the qubit frequency. When the optical frequencies are closely detuned from an optical transition in the atom, the beatnote drives two-photon Raman transitions. The beatnote can be generated in a number of ways. One way is to phase-lock two continuous-wave (CW) lasers and interfere them at the atom position. A more recent approach is to use the output of a mode-locked (ML) laser. The pulse train of an ML laser forms a comb of optical frequencies in frequency space, with each comb tooth separated by the repetition rate of the laser. By virtue of the mode-locking process, all comb teeth are phase coherent, and when the comb is split into two paths and interfered at the atom position, a series of beatnotes are generated. By placing a frequency shifter, such as an acousto-optical modulator, in one arm of the interferometer, beatnote harmonics can be finely tuned to the qubit frequency.

The number of different methods for driving atomic qubits with laser radiation, as well as the option to directly drive them with microwave radiation, necessitates a comparison of the influence of the method choice on qubit fidelities. While we find commonalities between each of the methods, the exact magnitude and spectral structure of laser noise can have a sizeable impact on qubit fidelities. Further, the choice of laser technology - whether it be the gain medium, or cavity design - can also limit achievable qubit control. The use of laser radiation to generate microwave beatnotes, rather than using microwaves directly, is typically motivated by the spatial specificity afforded by optical wavelengths. By focusing laser light down to the micron level, single atoms can be interrogated while minimally disturbing neighbouring qubits. Such a capability is essential for the realisation of universal quantum computation, as well as the arbitrary engineering of Hamiltonians in quantum simulations. Individual addressing with microwaves is possible using frequency specificity instead of spatial specificity, however such approaches typically require large magnetic field gradients to be generated near the atom positions. Laser radiation allows for such individual addressability to be performed universally over all atom trapping architectures using well known optical engineering techniques. 

In this paper we investigate the effect of realistic laser intensity and frequency noise on the fidelity of a primitive $\pi-$pulse between a ground and excited state in an ideal two-level atom. The fidelity of a $\pi-$pulse is chosen for ease of interpretation, and we note that fidelities of other common operations, such as a Ramsey sequence, are within an order of magnitude the same as the $\pi-$pulse for the same operation times. When using laser sources to generate the LO for qubit manipulation, the fundamental limiting factor becomes the spontaneous emission of the atomic states. For optical qubits driven by 1-photon transitions, this limit corresponds to the lifetime of the state used. For microwave qubits driven by 2-photon transitions, the spontaneous emission is from off-resonant scattering from the intermediate optical state. In this paper we calculate the infidelities of laser-driven qubit operations for realistic and state-of-the art laser technologies to quantify the necessary requirements for reaching the spontaneous emission (SE) fidelity floor. 

\subsection{Composite pulses}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{compositepulse_SSLvsDL.pdf}
    \caption{\textbf{The effect of two different laser sources, and two different control sequences on the qubit infidelity}, (a) The frequency noise PSD of a DPSSL and ECDL locked to a $1~$Hz reference over a $2\pi\times1~$MHz servo bandwidth, (b) The filter functions of a $\pi-$pulse and a composite SK1 pulse, with the duration of the SK1 pulse 5 times longer than the $\pi$-pulse (c) The infidelity of both a $\pi-$pulse and SK1 sequence for the two laser sources with Rabi frequency. The SNL in the laser source phase noise spectral densities is calculated through the typical required laser power to achieve each Rabi frequency. Region A is the SE floor of a 35 second lifetime optical qubit and region B is the SE floor for a two-photon Raman transition.}
    \label{fig:composite_pulse}
\end{figure}

Having outlined the limits to primitive operation fidelites from a linewidth-limited, and shot-noise limited laser source, it can be seen that frequency noise will typically be the limiting error from the laser source. Therefore, it is of interest to explore whether there exists more advanced control protocols for state transfer that are more resilient to laser frequency noise. It is well established that composite sequences of pulses can be designed that are more robust to static errors. The success in the correction of dynamic noise sources depends on the structure of the noise and here we investigate whether the structure of laser noise is amenable to composite pulse techniques. 

Filter function theory provides an intuitive way to understand the conditions under which a composite pulse sequence will correct for dynamic noise. In this picture, quantum operations are high pass filters on the phase noise spectrum such that low frequency noise contributes less to the operation error than the high frequency noise. Composite pulse sequences typically act as improved high-pass filters. The improved low frequency filtering is often at the expense of admitting more noise contributions around the Rabi frequency due to longer operation times. We therefore expect composite pulses to improve fidelities when high-frequency noise is a non-dominant contribution to the laser noise spectrum and to decrease fidelities when there is substantial high frequency noise. 

The contribution of high-frequency noise to the poor performance of composite pulse sequences has been previously shown for microwave oscillators \cite{ball2016role}. In Figure \ref{fig:composite_pulse} we calculate the errors due to frequency noise of a primitive gate and the composite pulse sequence SK1 for two different laser sources. Both sources have been linewidth narrowed to $1~$Hz with a servo bandwidth of $\wsrv=2\pi\times 1~$MHz, however one source is a DPSSL, and the other is an ECDL. The difference in relaxation oscillation frequencies between the two sources provides very different high frequency noise spectra, with the DPSSL falling to the SNL beyond the servo bandwidth, and the ECDL having excess phase noise (see Figure \ref{fig:composite_pulse}(a)). 

The operation errors for different Rabi frequencies are presented in Figure \ref{fig:composite_pulse}(c) and show a marked divergence in behaviour for the two laser sources. For the DPSSL, the increase in Rabi frequency moves the filter function higher in Fourier space such that less noise passes through. After the Rabi frequency exceeds the servo bandwidth the improved low frequency filtering of the SK1 pulse sequence improves on the linewidth-limited fidelity as the high frequency noise becomes non-dominant. For the ECDL, the fidelity initially matches the DPSSL (the high frequency noise is below the $\chi$-separation line) before diverging as the high frequency noise comes to dominate. Due to the increased susceptibility of SK1 to noise near the Rabi frequency compared to the primitive operation, it always performs the same, or worse, than the $\pi-$pulse. At Rabi frequencies above the servo bandwidth the ECDL reverts to its $h_b$-limited fidelity, as previously outlined. 

\section{Models of laser noise}

\subsection{Intensity noise}

To be more explict the RIN spectrum is defined as
\begin{equation}
S_\mathrm{RIN}(\omega) =
  \begin{dcases}
                                   A_w\frac{\omega_f}{\omega} & \text{for $\omega<\omega<\omega_f$} \\
  C \frac{A_w}{(1-(\omega/\omega_r)^2)^2 + A_r^{-1}} & \text{for $\omega>\omega_f$}
  \end{dcases}
  \label{eq:RIN}
\end{equation}
where $C=[(1-(\omega_f/\omega_r)^2)^2+A_r^{-1}]$ enforces continuity. The frequency $\omega_f$ is flicker corner frequency, and $\omega_r=2\pi/\tau_r$ is the relaxation frequency of the laser gain medium. The amplitude $A_w$ is the white noise amplitude, and $A_r$ is the amplitude of the relaxation peak above the white noise. To enforce the SNL all values of $S_\mathrm{RIN}(\omega)$ below the SNL are set to $S_\mathrm{SNL}$.

To calculate the effect of laser intensity noise on qubit control fidelities, we relate the RIN spectrum to the Rabi frequency noise spectrum. For optical transitions the relation is given by (see Methods)
\begin{equation}
    S_{\Omega,1\gamma}(\omega)=\frac{1}{4}S_\mathrm{RIN}(\omega)
\end{equation}
and for two-photon Raman transitions the laser intensity noise contributes twice such that
\begin{equation}
    S_{\Omega,2\gamma}(\omega)=S_\mathrm{RIN}(\omega)
\end{equation}

\subsection{Shot noise}

The shot noise of light is determined by the poisson statistics of photons, which sets a maximum signal to noise ratio (SNR) of an $N$ photon field of $N$/$\sqrt{N}$. For a detector of bandwidth $B$ the SNR is given by \cite{dakin2017handbook}
\begin{equation}
    \mathrm{SNR}=\frac{\bar{P}}{\delta P} = \sqrt{\frac{\bar{P}}{\hbar\omega_{O} B}}
\end{equation}
where $\bar{P}$ is the average power and $\delta P$ is the RMS power noise. The RMS noise can be related to the PSD of the laser RIN over a bandwidth $B$ as
\begin{equation}
    \frac{\delta P}{\bar{P}}=\sqrt{\frac{1}{2\pi}\int_0^B S_\mathrm{RIN}(\omega)d\omega}
\end{equation}
such that the shot noise limit of the PSD is given by
\begin{equation}
    S_\mathrm{RIN}(\omega)=\frac{2\pi\hbar\omega_{O}}{\bar{P}}
\end{equation}


\subsection{Frequency noise: optical}

The frequency noise spectral density of a free-running laser, $S^{(\mathrm{fr})}_{\delta\omega_\mathrm{LO}}$ typically follows the same structure as the RIN spectral density
\begin{equation}
S_\mathrm{\delta\omega_\mathrm{LO}}^\mathrm{(fr)}(\omega) =
  \begin{dcases}
     A_\mathrm{fr}\frac{\omega_f^\mathrm{(fr)}}{\omega} & \text{for $\omega<\omega_f^\mathrm{(fr)}$} \\
     C \frac{A_\mathrm{fr}}{(1-(\omega/\omega_r)^2)^2 + A_r^{-1}} & \text{for $\omega>\omega_f^\mathrm{(fr)}$}
  \end{dcases}
  \label{eq:frequency}
\end{equation}
At low frequencies, the spectrum is dominated by $1/f$-type noise before transitioning to a white noise floor. The amplitude of the white noise floor, $A_{fr}$, determines the intrinsic Lorentzian linewidth of the laser, however the linewidth is typically broadened above the intrinsic linewidth by the $1/f$ noise contributions \cite{stephan2005laser}. The technical linewidth of a laser source can be estimated by integrating all parts of the spectral density above the \emph{$\beta$-separation line}, defined as $S_{\delta\omega_{LO}}(\omega)>16\ln(2)\omega/\pi$ \cite{di2010simple}. Therefore, even though typical commercial laser sources have low intrinsic linewidths on the order of $0.1-1~$kHz, linewidth broadening from $1/f$ noise results in actual linewidths of $1~$kHz to $1~$MHz. Such linewidths are too incoherent to perform qubit rotations and therefore the $1/f$ noise must be suppressed below the $\beta$-separation line to perform quantum control of atomic transitions with laser sources.

In the same way that RIN spectral densities were related to the Rabi frequency noise spectral densities, the frequency and phase noise spectral densities can be related to a dephasing spectral density on the qubit as (see Methods)
\begin{equation}
    S_z(\omega)=\frac{1}{4}S_{\delta\omega_{LO}}(\omega)=\frac{1}{4}\omega^2S_{\phi}(\omega)
\end{equation}
such that the laser frequency and phase noise can be associated with a corresponding control error on the qubit.


\begin{table}
\caption{Typical laser intensity/frequency noise parameters for a diode laser (DL), diode-pumped solid-state laser (DPSS) https://www.osapublishing.org/ol/abstract.cfm?uri=ol-29-18-2148, modelocked fibre laser (MLFL). For the modelocked laser, the frequency noise of interest is in the repetition rate, and no relaxation oscillations are present.}
\begin{tabular}{lccc}

Parameter & DL & DPSS & MLFL \\ \hline
$\omega_f$ (Hz) & $2\pi\times10^4$ & $2\pi\times10^4$ & $<2\pi\times 10^3$\\ 
$A_w$ (dB/Hz) & SNL & -140 to -110 & -140 to -110 \\
$A_r$ (dB) & 10 to 30 & 10 to 30 & 0 to 10 \\
$\omega_r$ (Hz) & $2\pi\times10^9$ & $2\pi\times10^5$ & $2\pi\times 10^4$\\

\end{tabular}
\quad
\begin{tabular}{lccc}

Parameter & DL & DPSS & MLFL\\ \hline
$\omega_f$ (Hz) & $2\pi\times10^4$ & $2\pi\times10^4$ & $<2\pi\times 10^3$\\ 
 $A_{w}$ (dB/Hz) & 20 & -20 & 20 \\
$A_r$ (dB) & 10 to 30 & 10 to 30 & 0 to 10 \\
$\omega_r$ (Hz) & $2\pi\times10^9$ & $2\pi\times10^5$ & $2\pi\times 10^4$\\

\end{tabular}

\label{tab:laser_params}

\end{table}

\subsection{Frequency noise: microwave}

The driving of optical transitions with a single laser beam leads to the optical phase noise directly impinging on the qubit. When performing two-photon Raman transitions, common-mode phase noise cancels and it is the phase noise of the beatnote at the microwave frequency that is imprinted on the qubit. The importance is therefore in maximising the common-mode sources of phase noise. As we have already outlined, there are two common ways of driving Raman transitions
\begin{enumerate}
    \item Phase-lock two separate laser sources, offsetting the frequency of the two lasers by the qubit frequency using the phase-locked loop.
    \item Split the output of a mode-locked laser into two beams, offset one arm in frequency such that qubit transitions are driven using pairs of frequency comb teeth.
\end{enumerate}
A third, less common technique is sometimes used, which is to use an electro-optical modulator (EOM) to generate sidebands on an optical carrier frequency, which can then be used to drive Raman transitions directly. This method is typically limited in optical power due to the low damage thresholds of EOMs which can limit achievable Rabi frequencies. For this case of using a single laser source, the optical phase noise from the laser (ignoring mechanical and thermal effects) is entirely common-mode between the two arms. The contributions to the beatnote phase noise are then the phase noise in the modulator. Mechanical and thermal vibrations will contribute to anomalous phase noise in the beatnote, however in this paper we concentrate on noise contributions from optical and electronic sources. The phase noise due to a waveguide electro-optical modulator is on the order of -80 dB/Hz at 1 Hz \cite{barke2010eom}, such that the microwave oscillator driving the EOM would be the dominant contribution to the phase noise.

The use of two separate laser sources allows for greater optical power to be used for manipulating the qubit state than for the single laser with a modulator. The phase locking of the two individual lasers is performed in a similar way to the locking of a single laser to an optical cavity. A phase error signal is derived from the beat-note of the two lasers on a photodetector, which is fed back to the secondary laser such that its phase tracks that of the primary laser. The servo-loop again has a finite bandwidth, within which the suppression of frequency noise is given by the gain of the servo-loop, and outside of which the frequency noise is given by the mean of the two free-running frequency noise spectral densities

\begin{equation}
S_\mathrm{\delta\omega_{LO}}(\omega) =
  \begin{cases}
                                  A_s\omega_f/\omega & \text{for $\omega<\omega_f^{(s)}$} \\
                                  A_{s} & \text{for $\omega_f^{(s)}<\omega<\omega_s$} \\
  \frac{1}{2}\left(S_\mathrm{\delta\omega_{LO}}^{(fr,1)}(\omega) +S_\mathrm{\delta\omega_{LO}}^{(fr,2)}(\omega)\right) & \text{for $\omega>\omega_s$}
  \end{cases}
  \label{eq:servoedlaser}
\end{equation}
In the instance that the two lasers are identically prepared, such that $S_\mathrm{\delta\omega_{LO}}^{(fr,1)}(\omega)\approx S_\mathrm{\delta\omega_{LO}}^{(fr,2)}(\omega)$, then the power spectral density is equivalent to the case of a single laser locked to a cavity.

{\color{blue} Outline:}
{\color{blue} Resummarize the main results}

We find that qubit operations are high-pass filters on control noise. Lasers are low-pass filters on pump noise. Stabilization loops are high-pass filters on laser noise.

By playing with different filter parameters, we find that you can reach the spontaneous emission error floor. The relevant parameter is not the linewidth of the laser, but the details of the stabilized laser spectrum, with an interplay between 'effective linewidth' aka $h_a$, servo bandwidth, Rabi frequency, and residual high-frequency noise aka $h_b$. We present a simple relation between these parameters that defines whether and when residual high-frequency noise contributes significantly to qubit errors.

At a fundamental level, the frequency noise from the laser contributes more to errors than intensity noise from the laser. This holds even when we account for Stark shifts in addition to Rabi frequency noise. However, we do not account for beam pointing issues, which are a major cause of intensity noise in practice.


{\color{blue} Discuss the laser noise models(?)}

We investigated some caveats to the laser noise model presented earlier. Servo bumps do not substantially affect our results unless the servo bandwidth is close to the cutoff frequency. 

DPSSLs, however, do not follow the models presented because they typically exhibit $h_a>h_b$. 

We do not explicitly consider cases where the servo bandwidth is smaller than the relaxation peak, but not substantially smaller. However, our numerics indicate that in all cases we have investigated, the finding holds that spectral noise content above the chi separation line causes an increase in error rates above the fundamental limit.

{\color{blue} Discuss frequency noise stabilization requirements}

The tradeoff between the filter function order and the cutoff frequency seems to place some fundamental limits on the utility of composite pulse sequences.

In the frequency noise section, we found that the requirements on servo bandwidths are quite demanding, so we note that passive stabilization techniques may be preferable when feasible. One example of a passive stabilization technique is filtering the laser spectrum with a high-quality-factor optical resonator.

We find that  our results are applicable to mode-locked lasers, which differ from other laser sources considered primarily in the lack of a relaxation peak (and corresponding low-pass filtering of pump noise). However, these results indicate that you can't stabilize your way out of a noisy rep rate because the required servo bandwidths are prohibitive.

{\color{blue} Discuss intensity noise stabilization requirements}

Similar to frequency noise, there may be circumstances where passive stabilization is preferable for dealing with RIN and achieving shot-noise limited spectra. In such cases, one alternative might be the use of saturated optical amplifiers.

{\color{blue} How this will solve humanity's problems}

This work focuses on single qubit operations, but we envision a similar chi separation line could be derived for any Hamiltonian and filter function. 

{\color{blue} Left over text:}


{\color{red} One application of our work is to justify grant applications to making new DPSSL laser sources.} The finding that laser sources with low relaxation oscillations have a distinct advantage, allows for the identification of novel laser systems for high fidelity atomic qubit control. For example, for the long-lived the $1762~$nm quadrupole transition in Ba$^+$ there is no commercial DPSSL, with commercial ECDL sources restricted to fidelities of approximately $99.9\%$ after stabilisation. Thulium-doped glasses provide an ideal gain medium at this wavelength, and therefore the development of a diode-pumped, Tm-doped fiber laser with a frequency tuneable element in the laser cavity is of primary interest for high fidelity control of this transition. The long relaxation times of the Tm$^{3+}$ lasing process would act to filter out the high frequency diode noise. The models and analysis presented here allow for these identifications to be made for other atomic transitions.



{\color{red} Oh look you can generate microwave tones with mode-locked lasers. (part of the outlook?) (please note, lasers could therefore be relevant to SC qubits despite all appearance to the contrary)} These concepts from microwave sources are directly analogous to the frequency stabilisation of laser sources, where the variable oscillator takes the place of the laser source. Therefore, there is a requirement for the development of low noise variable oscillators for microwave synthesis such that qubit operations driven with microwave oscillators are not limited by high frequency noise. Such low noise oscillators could be generated using quantum-limited modelocked lasers, where tuning of the laser repetition rate would allow for variable microwave synthesis. The high frequency noise of microwaves synethesised from modelocked lasers is limited by the SNL, and the high power of these lasers means that fundamental noise floors of $<200~$dbc/Hz have been demonstrated. These shot-noise floors are below the thermal noise floor of crystal oscillators at 4K. Therefore, despite direct driving of atomic transitions with laser radiation being limited by spontaneous emission, the synthesis of microwave oscillators from laser radiation could provide a method for surpassing previously identified limits on the driving of qubit transitions with crystal oscillators. These results hold not only for atomic qubits, but also to sources for superconducting qubits.  

{\color{red} The simple model captures modelocked laser noise very well, but this makes stabilisation very challenging, and so pick a low noise laser}
{\color{gray} Modelocked lasers are a unique case, for which the simple model is a good approximation. As the LO is generated from a harmonic of the reptetition rate frequency, it's the jitter in the pulse-to-pulse timing that is important and not the optical frequency noise. In this instance, there is no low pass filter on the repetition rate frequency noise. Stabilisation of the LO frequency is limited by the stability of the microwave reference used, which in practice means that the value of $h_a$ can be low. Coupled with the fact that modelocked laser typically have high powers and drive qubit operations with high Rabi frequencies, the requirement on the servo bandwidth due to the $\chi-$separation line can get prohibitive. Therefore, for modelocked lasers it is imperative to select a laser with low free-running noise ($h_b$) as this will typically be the limiting factor. This also means that directly stabilising the repetition rate of the laser by having access to the cavity will not improve qubit fidelities, as it will be limited in its bandwidth to that of the thermal and mechanical actuators used.}


\section{Beatenote stabilisation in the PSD picture}

For the case where qubit transitions are driven with a frequency comb, then the residual phase noise is from variations in the repetition rate of the mode-locked laser. Here, each comb tooth can be thought of as a phase-locked oscillator, where the beat-note between each oscillator has a residual phase noise based on variations of the repetition rate of the pulsed laser. In practice, qubit transitions are driven between pairs of comb teeth that are separated approximately by the splitting of the qubit transition. It is therefore important to quantify the residual repetition rate noise between these comb teeth pairs. It has been found that the natural repetition rate noise of a free-space cavity mode-locked laser is too high for low-error qubit control, and therefore the beat note of the two comb teeth must be further stabilised to reduce the phase noise below the mode-locking phase noise. This is either done by stabilising the cavity length, or more easily, varying the modulator frequency that matches the two comb teeth to the atomic transition. More quantitatively the $n^\mathrm{th}$ harmonic beat note of two frequency combs of repetition rate $\omega_\mathrm{rep}$ can be tuned to the qubit drive frequency $\omega_\mathrm{q}$ using an AOM on one arm of the interferometer such that
\begin{equation}
    \omega_q=n \omega_\mathrm{rep} + \omega_\mathrm{AOM}
\end{equation}
where $\omega_\mathrm{AOM}$ is the drive frequency applied to the AOM. The repetition rate has an associated noise power spectral density $S^{(1)}_{\omega_\mathrm{rep}}(\omega)=S^{(1)}_{\phi_\mathrm{rep}}(\omega)/\omega^2$ such that the phase noise of the $m\mathrm{th}$ harmonic is given by
\begin{equation}
    S^{(m)}_{\phi_\mathrm{rep}}(\omega)=m^2 S^{(1)}_{\phi_\mathrm{rep}}(\omega)
\end{equation}
leading to an additional $20\log(m)$ phase noise in logarithmic units over the fundamental repetition rate phase noise. The phase noise associated with the repetition rate of the laser can be counteracted by applying a corrective drive frequency to the AOM. The action of driving the AOM is associated with its own phase noise, $S_{\phi_\mathrm{AOM}}(\omega)$ which becomes the limiting factor on the noise of the qubit drive frequency. The phase noise of an AOM is dominated by the microwave source used to drive the AOM. For simplicity we make the assumption that there is sufficient gain in the servo loop such that the in-loop phase noise is limited by the phase noise of the AOM driver. The phase noise cancellation can be performed by measuring any of the $m$ harmonic beatnotes and feeding back to the AOM driver such that the beatnote lock phase noise spectral density is given by
\begin{equation}
    S^{(m)}_{\mathrm{BNL}}(\omega)=
  \begin{cases}
  S_{\phi_\mathrm{AOM}}(\omega) & \text{for $\omega<\omega_s$} \\
  S^{(m)}_{\phi_\mathrm{rep}}(\omega) & \text{for $\omega>\omega_s$} 
  \end{cases}
\end{equation}
where $\omega_s$ is the bandwidth of the servo-loop used to perform the beatnote lock. In general, if the beatnote lock is performed on the $m^\mathrm{th}$ harmonic then the phase noise at the qubit frequency harmonic, $n$, is given by
\begin{equation}
S_{\phi_q}(\omega)=\frac{n^2}{m^2} S^{(m)}_{\mathrm{BNL}}(\omega)
\end{equation}
such that the noise of the beatnote lock is amplified by $20\log(n/m)$ at the qubit frequency. It would therefore appear advantageous to lock the beatnote at the $n^\mathrm{th}$ harmonic, however the phase noise of the microwave oscillator has to be carefully considered. The majority of tuneable microwave drivers are upconverted from a fundamental clock frequency. As these clock frequencies are of the same order of magnitude as typical repetition rates, the upconversion noise of the microwave source to the $n^\mathrm{th}$ harmonic can be of the same order as the upconversion noise of the optical beatnote. It is therefore of critical importance to assess the difference in these two upconversion processes to generate the cleanest beatnote frequency. A better way is to use a source with a natural clock frequency at the typical $\sim10~$GHz microwave qubit frequencies, such as a sapphire oscillator. While these sources typically have higher phase noise than sources in the $10~$MHz range, they are of lower noise than an upconverted $10~$MHz signal - providing an advantage in the resulting beatnote phase noise if enough servo gain can be achieved. While a precise analysis of servo loop design for beatnote locking is beyond the scope of this paper, we note that signal-to-noise ratio will most likely be the primary determinant of which harmonic to lock to. At the fundamental harmonic, the phase noise may be so low that it is below the detection floor. At higher harmonics, the response of the detector may limit the recorded signal.

 The field of optical microwave synthesis offers a signpost to the generation of low-noise microwave beatnotes at atomic qubit frequencies \cite{cundiff2001optical}. Microwave signals generated with optical beatnotes of modelocked lasers can now surpass those of commercial microwave oscillators \cite{xie2017photonic}, opening up the possibility of driving high fidelity quantum operations without beatnote stabilisation. In this instance, the phase noise of the AOM driver becomes the limiting error source. However, by synthesising a microwave beatnote from the frequency comb, the AOM driver could be phase-locked to the comb, thereby limiting the fidelity floor to the repetition rate variations of the comb. 
 
 \section{Modulation index theory for determining laser linewidth}


 
 \section{Linewidth to timing jitter conversion}

Consider a modelocked laser with a linewidth of $\Delta^{(m)}_\mathrm{FWHM}$ at the $m$th harmonic of the frequency comb such that the frequency noise PSD is given by
\begin{equation}
    S^{(m)}_{\nu_\mathrm{rep}}(f)=\frac{\Delta^{(m)}_\mathrm{FWHM}}{\pi}
\end{equation}
such that
\begin{equation}
    S^{(1)}_{\nu_\mathrm{rep}}(f)=\frac{\Delta^{(m)}_\mathrm{FWHM}}{\pi m^2}=\frac{\Delta^{(1)}_\mathrm{FWHM}}{\pi}
\end{equation}
The timing jitter of the fundamental harmonic is given by integrating over the phase noise $S^{(1)}_{\phi_\mathrm{rep}}(f)=S^{(1)}_{\nu_\mathrm{rep}}(f)/f^2$ to obtain
\begin{equation}
    \delta_t=\frac{1}{2\pi \nu_\mathrm{rep}}\sqrt{2\int_{f_\mathrm{min}}^{f_\mathrm{max}} \frac{S^{(1)}_{\nu_\mathrm{rep}}(f)}{f^2} df}=\frac{1}{2\pi \nu_\mathrm{rep}}\sqrt{2\int_{f_\mathrm{min}}^{f_\mathrm{max}} \frac{\Delta^{(m)}_\mathrm{FWHM}}{\pi m^2 f^2} df}
\end{equation}
where $f_\mathrm{min}$ is typically chosen as $10~$Hz and $f_\mathrm{max}=\nu_\mathrm{rep}$ is the Nyquist frequency. The timing jitter can now be connected to the linewidth at the $m$th harmonic closest to the qubit frequency. For the numbers in the manuscript we used $\nu_\mathrm{rep}=100~$MHz and $m=100$.

\section{AC Stark shift constants}



\section{Non-ideal laser noise PSDs}

\subsection{Servo bumps}\label{app:servo_bumps}



\subsection{Spurs}

{\color{red}\subsection{Laser noise models}

 In order to make generalizable conclusions on the effect of laser noise on atomic qubit control, we use toy models of laser noise motivated by physical processes present in lasers. The models are defined in the frequency domain as power spectral densities, as are commonly presented in the literature for both laser noise measurements, as well as theoretical laser noise models. We investigate both intensity noise and frequency (phase) noise separately to study their independent limits on qubit fidelities.

\subsubsection{Intensity noise}

The power spectral density of relative intensity noise (RIN), $S_\mathrm{RIN}(\omega)$, can be divided into four main regimes, as shown in Figure \ref{fig:laser_noise_models}(a). At low frequencies, RIN is dominated by noise in the electronics used to drive the laser source. The electronic noise is converted into optical noise due to the dependence on the optical power on the electronic power. The electronic noise consists of $1/f$-type noise at the lowest frequencies (region I) before transitioning to white noise given by the thermal noise floor of the electronics (region II). For simplicity we assume the electronic noise assumes a $1/\omega^1$ noise (flicker, or pink, noise). Other contributions, such as $1/\omega^2$ noise (Brownian, or red, noise) are not considered here as their effect for typical laser parameters was found to be negligible. At the flicker corner frequency, the flicker noise transitions to $1/\omega^0$, or white, noise that is constant with Fourier frequency. For sufficiently low electronic noise, the white noise amplitude is instead limited by the shot-noise limit of the laser light, defined as $S_\mathrm{SNL}=2h\omega_\mathrm{LO}/\bar{P}$ where $\omega_\mathrm{LO}$ is the optical carrier frequency and $\bar{P}$ is the time-averaged power that the RIN is defined with respect to.

At high Fourier frequencies, the RIN spectrum is dominated by the relaxation dynamics of the laser medium. At the inverse of the upper-state lifetime of the gain medium, the RIN features a Lorentzian peak due to relaxation oscillations (region III). Above the relaxation peak, the intensity noise decays down to the shot-noise limit (region IV). The maximum Fourier frequency is given by the control bandwidth, thereby ensuring that the noise remains finite.

 A representative RIN model is shown in Figure \ref{fig:laser_noise_models}(a).

The toy model of RIN given by Equation \ref{eq:RIN} can capture the dynamics of laser noise in all laser technologies by appropriate choice of model parameters. We list typical values of these parameters in Table \ref{tab:itensity_noise_params}. Semiconductor diode lasers are electrically driven and, with appropriate choice of low-noise electronics, exhibit flicker corner frequencies of approximately $10~$kHz, with electronic thermal noise floors at, or below, the SNL of the laser light. The upper state lifetimes of laser diodes are on the order of $\sim1~$ns and therefore have relaxation frequencies in the GHz range. Solid-state lasers use a doped gain medium (such as Ti:Sapphire) that is optically pumped, typically by a diode laser. Solid-state gain mediums typically have long upper-state lifetimes and exhibit relaxation frequencies in the $100~$kHz range. Below the relaxation peak the RIN of the pump laser is amplified by the gain medium, and above the relaxation peak the pump noise is effectively filtered out. Therefore when using diode lasers to pump solid-state gain media, the relaxation oscillations of the diode are filtered from the resulting laser light, and the electronically generated optical noise of the diode laser is the dominant noise source. Mode-locked lasers are typically composed of solid-state gain media, and therefore have similar characteristics.

\begin{table}
\caption{Typical laser intensity noise parameters for a diode laser (DL), solid-state laser (SL), modelocked fibre laser (MLFL)}

\begin{tabular}{lccc}

Parameter & DL & SSL & MLFL \\ \hline
$\omega_f$ (Hz) & $2\pi\times10^4$ & $2\pi\times10^4$ & $<2\pi\times 10^3$\\ 
$A_w$ (dB/Hz) & SNL & -140 to -110 & -140 to -110 \\
$A_r$ (dB) & 10-30 & 10-30 & 0-10 \\
$\omega_r$ (Hz) & $2\pi\times10^9$ & $2\pi\times10^5$ & $2\pi\times 10^4$\\

\end{tabular}
\label{tab:itensity_noise_params}
\end{table}

To calculate the effect of laser intensity noise on qubit control fidelities, we relate the RIN spectrum to the Rabi frequency noise spectrum. For optical transitions the relation is given by (see Methods)
\begin{equation}
    S_{\Omega,1\gamma}(\omega)=\frac{1}{4}S_\mathrm{RIN}(\omega)
\end{equation}
and for two-photon Raman transitions the laser intensity noise contributes twice such that
\begin{equation}
    S_{\Omega,2\gamma}(\omega)=S_\mathrm{RIN}(\omega)
\end{equation}

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{LaserNoiseModels.pdf}
    \caption{Example power spectral densities of (a) relative intensity noise demonstrating regions of (I) flicker noise (II) white noise (III) relaxation noise (IV) shot noise, (b) frequency noise, with regions of (I) flicker noise (II) servoed white noise (III) free-running frequency noise (IV) relaxation noise, the blue dashed line indicates the $\beta$-separation line, (c) the equivalent phase noise of (b) with the additional region of (V) shot noise.}
    \label{fig:laser_noise_models}
\end{figure}

\subsubsection{Frequency and Phase noise of optical LOs}

The frequency noise spectral density of a free-running laser, $S^{(\mathrm{fr})}_{\delta\omega_\mathrm{LO}}$ typically follows the same structure as the RIN spectral density
\begin{equation}
S_\mathrm{\delta\omega_\mathrm{LO}}^\mathrm{(fr)}(\omega) =
  \begin{dcases}
     A_\mathrm{fr}\frac{\omega_f^\mathrm{(fr)}}{\omega} & \text{for $\omega<\omega_f^\mathrm{(fr)}$} \\
     C \frac{A_\mathrm{fr}}{(1-(\omega/\omega_r)^2)^2 + A_r^{-1}} & \text{for $\omega>\omega_f^\mathrm{(fr)}$}
  \end{dcases}
  \label{eq:frequency}
\end{equation}
At low frequencies, the spectrum is dominated by $1/f$-type noise before transitioning to a white noise floor. The amplitude of the white noise floor, $A_{fr}$, determines the intrinsic Lorentzian linewidth of the laser, however the linewidth is typically broadened above the intrinsic linewidth by the $1/f$ noise contributions \cite{stephan2005laser}. The technical linewidth of a laser source can be estimated by integrating all parts of the spectral density above the \emph{$\beta$-separation line}, defined as $S_{\delta\omega_{LO}}(\omega)>16\ln(2)\omega/\pi$ \cite{di2010simple}. Therefore, even though typical commercial laser sources have low intrinsic linewidths on the order of $0.1-1~$kHz, linewidth broadening from $1/f$ noise results in actual linewidths of $1~$kHz to $1~$MHz. Such linewidths are too incoherent to perform qubit rotations and therefore the $1/f$ noise must be suppressed below the $\beta$-separation line to perform quantum control of atomic transitions with laser sources.

\begin{table}
\caption{Typical laser frequency noise parameters for a diode laser (DL), solid-state laser (SL), modelocked fibre laser (MLFL). For the modelocked laser, the frequency noise of interest is in the repetition rate, and no relaxation oscillations are present.}

\begin{tabular}{lccc}

Parameter & DL & SSL & MLFL\\ \hline
$\omega_f$& $2\pi\times10^4$ & $2\pi\times10^4$ & $<2\pi\times 10^3$\\ 
 $A_{fr}$ & 10^2 & ? & 10^2 \\
$A_r$ & 10-30 dB & 10-30 dB & -\\
$\omega_r$ & $2\pi\times10^9$ & $2\pi\times10^5$ & -\\

\end{tabular}

\end{table}

\begin{table}
\caption{Typical laser intensity/frequency noise parameters for a diode laser (DL), diode-pumped solid-state laser (DPSS) https://www.osapublishing.org/ol/abstract.cfm?uri=ol-29-18-2148, modelocked fibre laser (MLFL). For the modelocked laser, the frequency noise of interest is in the repetition rate, and no relaxation oscillations are present.}
\begin{tabular}{lccc}

Parameter & DL & DPSS & MLFL \\ \hline
$\omega_f$ (Hz) & $2\pi\times10^4$ & $2\pi\times10^4$ & $<2\pi\times 10^3$\\ 
$A_w$ (dB/Hz) & SNL & -140 to -110 & -140 to -110 \\
$A_r$ (dB) & 10 to 30 & 10 to 30 & 0 to 10 \\
$\omega_r$ (Hz) & $2\pi\times10^9$ & $2\pi\times10^5$ & $2\pi\times 10^4$\\

\end{tabular}
\quad
\begin{tabular}{lccc}

Parameter & DL & DPSS & MLFL\\ \hline
$\omega_f$ (Hz) & $2\pi\times10^4$ & $2\pi\times10^4$ & $<2\pi\times 10^3$\\ 
 $A_{w}$ (dB/Hz) & 20 & -20 & 20 \\
$A_r$ (dB) & 10 to 30 & 10 to 30 & 0 to 10 \\
$\omega_r$ (Hz) & $2\pi\times10^9$ & $2\pi\times10^5$ & $2\pi\times 10^4$\\

\end{tabular}

\label{tab:laser_params}

\end{table}

Laser linewidth narrowing is typically performed by monitoring frequency deviations of a laser with respect to a stable reference, such as a high-finesse cavity. A servo loop is used that takes as input an error signal, derived from deviations of the laser frequency from the reference, and outputs a control signal to the laser (for example, the current of a laser diode). The gain profile of the servo loop must be carefully designed to suppress the free-running laser noise. The servo bandwidth, $\omega_s$, is the maximum Fourier frequency for which the free running noise is reduced by the servo loop, that is the frequency at which the gain reaches unity. The maximum allowable servo bandwidth is determined by either the stability of the loop, the time delay of the servo electronics, or the response bandwidth of the feedback actuator - with typical values of $\omega_s$ of $2\pi\times 100~$kHz to $2\pi\times 6~$MHz.

For simplicity, we assume that the servo gain profile has been well-designed such that the servoed laser has a constant frequency noise amplitude, $A_s$, below the servo bandwidth, and reverts to its free-running noise amplitude $A_{fr}$ above the servo bandwidth. The smallness of $A_s$ is fundamentally limited by thermal noise of the high-finesse cavity, which contributes a $1/f$-type contribution at the lowest Fourier frequencies. The full frequency spectral density is therefore expressed
\begin{equation}
S_\mathrm{\delta\omega_{LO}}(\omega) =
  \begin{cases}
                                  A_s\omega_f/\omega & \text{for $\omega<\omega_f^{(s)}$} \\
                                  A_{s} & \text{for $\omega_f^{(s)}<\omega<\omega_s$} \\
  S_\mathrm{\delta\omega_{LO}}^{(fr)}(\omega) & \text{for $\omega>\omega_s$}
  \end{cases}
  \label{eq:servoedlaser}
\end{equation}
The minimum required servo bandwidth to reduce the linewidth of the laser from the free-running linewidth is set by the requirement for the free-running noise amplitude to be completely below the $\beta$-separation line
\begin{equation}
    \omega_s^\textrm{min,$\beta$}=\frac{ S_\mathrm{\delta\omega_{LO}}^{(fr)}(\omega>\omega_s)}{32\ln(2)}
\end{equation}
such that the linewidth of the servoed laser is given by $\Gamma_s\approx A_s/(4\pi)$ \cite{di2010simple}. An example spectral density of a servoed diode laser is shown in Figure \ref{fig:laser_noise_models}(b), where the free-running noise immediately above the servo bandwidth is given by the free-running white noise floor. The increase in white noise amplitude, from the servoed value, to the free-running value is referred to as the \emph{servo-bump} as it leads to sidebands on the laser lineshape at the servo frequency. The step-change from servoed- white noise level to free-running white noise is an approximation of our model. In practice, the transition is smooth, and can often exhibit a peak of amplified noise at the servo bandwidth. We address the validity of the step-model approximation when calculating fidelity values below. For solid state lasers the relaxation oscillation peak is low enough that it can be suppressed by a well-designed servo gain profile such that the free-running noise above the servo bandwidth is simply the shot noise limit. Therefore, for solid-state lasers with $\omega_s>\omega_r$, servo-bumps are typically not observed.

The frequency spectral density can be related to the phase spectral density by
$S_{\phi}(\omega)=S_{\delta\omega_{LO}}(\omega)/\omega^2$. The advantage of representing frequency noise in phase space is that the shot-noise limit is well defined. In our analysis we set any values of $S_{\phi}(\omega)$ below the SNL to be equal to the $S_\mathrm{SNL}$. An example phase spectral density is shown in Figure \ref{fig:laser_noise_models}(c).

In the same way that RIN spectral densities were related to the Rabi frequency noise spectral densities, the frequency and phase noise spectral densities can be related to a dephasing spectral density on the qubit as (see Methods)
\begin{equation}
    S_z(\omega)=\frac{1}{4}S_{\delta\omega_{LO}}(\omega)=\frac{1}{4}\omega^2S_{\phi}(\omega)
\end{equation}
such that the laser frequency and phase noise can be associated with a corresponding control error on the qubit.

\subsubsection{Frequency and phase noise of beatnote LOs}

 
 \subsubsection{Intensity-noise to frequency-noise conversion}

For off-resonant excitation of atomic transitions, the time-varying electric field causes energy level shifts due to AC stark shifts. The strength of the AC stark shift depends on the magnitude of the electric field strength, and therefore on the light intensity at the position of the atom. Therefore, variations of the intensity of the laser beam will cause variations in the frequency of the atomic transition, leading to an effective dephasing term in the Hamiltonian. For Raman transitions driven by two CW laser beams of equal intensity, $I$, the frequency shift is directly proportional to $I$ and as such the power spectral density of the AC stark shift can be written (see Methods)
\begin{equation}
    S_\mathrm{AC}^\mathrm{(cw)}=\left(\mu_\mathrm{cw} \frac{\Omega_{2\gamma}}{2}\right)^2 S_\mathrm{RIN}
\end{equation}
where $\Omega_{2\gamma}$ is the two-photon Rabi frequency and $\mu_{cw}$ depends on the detuning of the radiation from closely detuned energy levels. The value of $\mu_{cw}$ is typically on the order of $1\times10^{-4}$. 

The driving of Raman transitions with a frequency comb leads to an additional AC stark shift contribution. Each comb tooth contributes to the stark shift, amplifying its effect. The resulting intensity-to-frequency noise conversion takes the form (see Methods)
\begin{equation}
    S_\mathrm{AC}^\mathrm{(fc)}=\left(\mu_\mathrm{fc} \Omega'_{2\gamma}^2\right)^2 S_\mathrm{RIN}
\end{equation}
where $\Omega'_{2\gamma}$ is the two-photon Rabi frequency taking into account the finite pulse length of the frequency comb, and $\mu_\mathrm{fc}$ depends on the comb spacing and detuning of the comb from closely detuned transitions. The value of $\mu_{fc}$ is typically on the order of $1\times10^{-8}$. 





}

\section{Spare text snippets}

Fidelities of primitive operations under the influence of dephasing noise calculated by filter function theory were validated by comparison to a brute-force numerical evolution of the Shrodinger equation. The simulations were performed in the time domain, and random noise fields due to laser noise were generated from their respective power spectral densities. Ensembles of evolutions were performed and then averaged to obtain the probability of finding the qubit in the correct state under the influence of the noise field.

\subsection{Spectral density theory}

We assume the noise fields are stationary, independent, non-Markovian, and have zero mean such that a noise field $\beta_y(t)$ can be related to its single-sided power spectral density through the Weiner-Khinchin theorem as
\begin{equation}
\langle\beta_y(t_1)\beta_y(t_2)\rangle=\frac{1}{\pi}\int^\infty_{0} S_y(\omega)e^{i\omega(t_2-t_1)}d\omega
\end{equation}
where $\langle\cdot\rangle$ denotes time-averaging of the random variables. Further, we express the noise field as $\beta_y=\alpha\delta f_y(t)$ where $\alpha$ is constant in time. Through the linearity of the time-averaging operation
\begin{align}
\langle\beta_y(t_1)\beta_y(t_2)\rangle&=\alpha^2\langle\delta f_y(t_1)\delta f_y(t_2)\rangle \\
&=\frac{\alpha^2}{\pi}\int^\infty_{0} S_{f_y}(\omega)e^{i\omega(t_2-t_1)}d\omega
\end{align}
such that $S_y(\omega)=\alpha^2 S_{f_y}(\omega)$. The relationships between the spectral density of the noise fields, $S_z$ and $S_\Omega$ can therefore be related to the laser noise spectral densities through the relationship of $\beta_z$ and $\beta_\Omega$ to the laser parameters $\delta I/I$ and $\delta\omega_{LO}$.

\subsection{Filter function theory}

Under the assumption of small noise amplitudes, the fidelity of a unitary quantum operation of length $\tau$ can be related to the spectral densities of the noise fields by
\begin{equation}
 \mathcal{F}^{(u)}(\tau)=\frac{1}{2}\left\{1+\exp[-\chi^{(u)}(\tau)]\right\}   
\end{equation}
with
\begin{equation}
    \chi^{(u)}(\tau)=\frac{1}{\pi}\int_0^\infty \frac{d\omega}{\omega^2} S_z(\omega) F_z^{(u)}(\omega) + \frac{1}{\pi}\int_0^\infty \frac{d\omega}{\omega^2} S_\Omega(\omega) F_\Omega^{(u)}(\omega) 
\end{equation}
where $F_z^{(u)}(\omega)$ and $F_\Omega^{(u)}(\omega)$ are the filter functions of the quantum operation. For a $\pi$-pulse around $X$ the dephasing filter function is given by
\begin{equation}
F^{(\pi)}_z(\omega)=\left\lvert \frac{\omega^2}{\omega^2 - \Omega^2} (e^{i\omega\tau_\pi} + 1)\right\rvert^2+\left\lvert \frac{i\omega\Omega}{\omega^2 - \Omega^2} (e^{i\omega\tau_\pi} + 1)\right\rvert^2
\label{eq:prim_filter}
\end{equation}
where $\tau_\pi=\pi/\Omega$. By Taylor expanding $F^{(\pi)}_z(\omega)$ and taking the leading order, $F^{(\pi)}_z(\omega)$ can be approximated by the piecewise function
\begin{equation}
    F^{(\pi)}_{z}(\omega)\approx
  \begin{cases}
  4\omega^2/\Omega^2 & \text{for $\omega<\Omega$} \\
  4 & \text{for $\omega>\Omega$} 
  \end{cases}
\end{equation}
such that the approximate analytic fidelity in Equation (\ref{eq:fidelity_servo}) can be derived. The filter functions for amplitude noise do not have a closed analytic form, and are calculated numerically.



\subsection{Spare text}

Making the identification $\delta\Omega_c=\beta_\Omega(t)\Omega_c(t)$ the amplitude noise field can be expressed in terms of the relative intensity noise as
\begin{equation}
\beta_{\Omega,1\gamma}(t)=\sqrt{1+\frac{\delta I(t)}{I}}-1\approx\frac{1}{2}\frac{\delta I(t)}{I}
\end{equation}

such that it can be directly identified that
\begin{equation}
\beta_{\Omega,2\gamma}(t)=\frac{\delta I(t)}{I}
\end{equation}

\subsection{Lasers as Local Oscillators}


\section{Sections to be Incorporated}



\section{Intensity noise details}

\begin{figure*}
    \centering
    \includegraphics[width=0.8\linewidth]{IntensityNoiseFidelity_v3.pdf}
    \caption{\textbf{The influence of free-running and servoed ($\wsrv=2\pi\times3~$MHz) laser intensity noise on qubit errors for realistic ECDL (blue) and DPSSL (red) sources}. The SNL is determined by the required power for each Rabi frequency for Ba$^+$ optical and microwave qubits. (a) ECDL intensity noise spectrum with Rabi frequency for carrier transitions demonstrating that shot noise dominates at low $\Omega$ and technical laser noise dominates at high $\Omega$. Servoed intensity is shown with transparency. (b) DPSSL free-running (solid) and servoed (transparent) intensity noise spectrum with Rabi frequency, (c) Comparison of the error from intensity noise to the SE floor demonstrating that technical laser noise can cause qubit errors to exceed the SE floor. Active servo suppression of intensity noise is effective for DPSSL but not ECDL sources. (d-f) Equivalent plots for Raman transitions. }
    \label{fig:intensity_noise}
\end{figure*}

{\color{red} By the way, you have heard of intensity stabilization as noise eating.}
In the context of intensity noise the stabilisation is often referred to as noise-eating. 
High bandwidth noise-eating can be performed using an AOM on the laser output \cite{zhao2017gain,wang2020reduction}.

{\color{red} For Raman transitions, the shot noise limit is always below the spontaneous emission limit regardless of the Rabi frequency.} 
For Raman transitions, the required power to drive a $\pi-$pulse in a single-valence electron atom is given by a combination of atomic and laser properties \cite{ozeri2007errors}
\begin{equation}
P_{2\gamma}=\frac{2\pi}{3\epsilon_{SE,2\gamma}}\left(\frac{2\pi w_0}{\lambda_{3/2}}\right)^2\hbar \omega_{3/2} \Omega_{2\gamma}~,
\label{eq:ramanpower}
\end{equation}
where $\epsilon_{SE,2\gamma}$ is the error from spontaneous emission, depending on the laser detuning and atomic fine structure (see Methods), $\lambda_{3/2}=c/\omega_{3/2}$ is the wavelength of the $S_{1/2}\rightarrow P_{3/2}$ transition and $w_0$ is the beam radius at the atom position. 
Setting $h_a$ to be the SNL and using Equation \ref{eq:ramanpower}, we find that the requirement on the laser intensity noise reduces to one on the numerical aperture of the addressing beam such that
\begin{equation}
\mathrm{NA}<4\sqrt{\frac{\pi}{3}}\approx 4~,
\end{equation}
where $\mathrm{NA}=\lambda_O/(\pi w_0)$ is the numerical aperture, $\lambda_{O}$ is the wavelength of the laser light, and the approximation of $\lambda_{O}\approx\lambda_{3/2}$ sets a stricter bound as typically $\lambda_{O}<\lambda_{3/2}$. 
Therefore the error from SNL laser light addressing Raman transitions is always below the error from spontaneous emission up to the Abbe limit of $\mathrm{NA}=1$ in vacuum.

{\color{red} Requirement reduces to NA$<$0.77; more strict but easily achievable in practical applications

shot noise limit higher than for Raman because the transition is more 'efficient' 

Both spontaneous emission error (propto intensity) and shot noise (propto power) scale the same with Rabi frequency and we can tune their relative magnitudes with the beam waist (ie the NA).} 
For optical transitions, the required power to drive Rabi oscillations in a quadrupole transition is given by (see Supplementary Materials)
\begin{equation}
P_{1\gamma} = \frac{8\pi^3\hbar c}{5\Gamma\lambda_O^3}w_0^2\Omega_{1\gamma}^2~,
\end{equation}
where $\Gamma=1/{\tau_e}$ is the decay rate of the excited state. 
The resulting constraint on the numerical aperture
\begin{equation}
    \mathrm{NA}<\sqrt{\frac{6\pi}{5}}\approx 2~,
\end{equation}
where we have used the expression $\epsilon_{SE,1\gamma}=3\pi/(8\Omega\tau_e)$ (see Methods).
The constraint on the numerical aperture is tighter than for Raman transitions and is not satisfied up to the Abbe limit. 
The primary reason for this is that optical transitions are more efficient, requiring less laser power and higher shot noise limits.
However we note that the limit corresponds approximately to $\mathrm{NA}<0.77$ which covers typical addressing optical set ups.

\begin{figure*}[!h]
    \centering
    \includegraphics[width=1\linewidth]{servo_bump_compare.pdf}
    \caption{(a) The infidelity of a servoed diode laser due to a servo bump, compared to the simple model assumed in the main text with (dotted) corresponding to the spectra shown in (b) and (dashed) corresponding to the spectra shown in (c). (b-c) Cropped plots of the laser noise spectra with (dot-dashed) indicating the Rabi frequency used in (a).}
    \label{fig:servo_bump_comparison}
\end{figure*}

In our analysis, the models of laser noise were chosen for ease of interpretation. However, in physical laser noise spectra there are spurs and bumps in the noise spectrum. Here we include a common bump in laser noise spectra, the one caused by the servo loop close to the servo bandwidth. To model this feature, we place a Lorentzian peak at the servo bandwidth, with a peak amplitude $20~$dB higher than the out-of-loop white noise level. In Figure \ref{fig:servo_bump_comparison}(a) we plot the infidelity of a primitive operation for different servo bandwidths and a fixed Rabi frequency. At the $\chi-$separation line (dashed line) we find a neglible increase in the error due to the presence of slightly increased higher frequency noise - however the $\chi-$separation line still indicates the point at which the infidelity trends to the linewidth-limited value. For servo bandwidths very close to the Rabi frequency a significant increase in error is observed due to the bump not being effectively filtered by the quantum operation. Therefore, for realistic laser noise spectra that include servo bumps, the servo bandwidth should be placed as far above the Rabi frequency as possible - ideally at the $\chi-$separation line.

\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{modulation_index.pdf}
    \caption{The predicted linewidth of laser radiation as a function of the cut-off modulation index, $\beta_c$, included in the calculation. For $\beta_c<1$ (indicated by dashed line) the linewidth is constant, demonstrating that noise with low modulation index does not contribute to the linewidth. }
    \label{fig:modulation_index}
\end{figure}

\subsection{Requirements on laser noise to reach the spontaneous emission floor}

Having derived the fidelity from simplified laser noise PSD we compare the error from laser noise to the error from spontaneous emission. Assume the error from SE is given by $\epsilon_\mathrm{SE}$ then we have the requirement
\begin{equation}
\epsilon_\mathrm{SE}>\chi^{(u)}(\tau)/2=\frac{H^{(u)}_b}{8\pi}\left[ \frac{n}{n-1} \frac{h_a}{\omega_c}  +  \frac{h_b-h_a}{\omega_s}\right]
\end{equation}
Rearranging for $h_a$ we find
\begin{equation}
h_a<\frac{1}{\frac{n \omega_s}{(n-1)\omega_c} -1}\left(\frac{8\pi\epsilon_\mathrm{SE}\omega_s}{H_b^{(u)}} - h_b\right)
\end{equation}
which sets the requirement $\omega_s>(n-1)\omega_s/n$ and $h_b<8\pi\epsilon_\mathrm{SE}\omega_s/H_b^{(u)}$ in order for $h_a>0$. The condition for $h_b$ shows that it can tend to infinity as the servo bandwidth tends to infinity.

Rearranging for the servo bandwidth instead we find
\begin{equation}
\omega_s>\frac{1}{\frac{8\pi\epsilon_\mathrm{SE}}{H_b^{(u)} h_a}-\frac{n}{(n-1)\omega_c}}\left(\frac{h_b}{h_a}-1\right)
\end{equation}
which is a more restrictive version of the general requirement on the servo bandwidth to maximise fidelity. From this expression we see that $h_a<(n-1)8\pi\epsilon_\mathrm{SE}\omega_c/(nH_b^{(u)})$ which sets a minimum value of $h_a$ such that a servo bandwidth can be used (i.e. it is the value for infinite servo bandwidth).

Summarising these conditions for a $\pi$-pulse:
\begin{align}
h_a&<\frac{1}{\frac{2 \omega_s}{\Omega} -1}\left(2\pi\epsilon_\mathrm{SE}\omega_s - h_b\right)\\
\omega_s&>\frac{1}{\frac{2\pi\epsilon_\mathrm{SE}}{h_a}-2/\Omega}\left(\frac{h_b}{h_a}-1\right) \\
h_a&<\pi\epsilon_\mathrm{SE}\Omega
\end{align}
For $\epsilon_\mathrm{SE}=10^{-6}$ and $\Omega=10^6$ we find $h_a<\pi$, which at infinite bandwidth corresponds to an effective linewidth of $1/4$ Hz
